PRISM: Breaking the O(n) Memory Wall in Long-Context LLM Inference via O(1) Photonic Block Selection

Long-context LLM inference is bottlenecked not by compute but by the O(n) memory bandwidth cost of scanning the KV cache at every decode step -- a wall that no amount of arithmetic scaling can break. Recent photonic accelerators have demonstrated impressive throughput for dense attention computation; however, these approaches inherit the same O(n) memory scaling as electronic attention when applied to long contexts. We observe that the real leverage point is the coarse block-selection step: a memory-bound similarity search that determines which KV blocks to fetch. We identify, for the first time, that this task is structurally matched to the photonic broadcast-and-weight paradigm -- the query fans out to all candidates via passive splitting, signatures are quasi-static (matching electro-optic MRR programming), and only rank order matters (relaxing precision to 4-6 bits). Crucially, the photonic advantage grows with context length: as N increases, the electronic scan cost rises linearly while the photonic evaluation remains O(1). We instantiate this insight in PRISM (Photonic Ranking via Inner-product Similarity with Microring weights), a thin-film lithium niobate (TFLN) similarity engine. Hardware-impaired needle-in-a-haystack evaluation on Qwen2.5-7B confirms 100% accuracy from 4K through 64K tokens at k=32, with 16x traffic reduction at 64K context. PRISM achieves a four-order-of-magnitude energy advantage over GPU baselines at practical context lengths (n >= 4K).

==> sections/crossover.tex <==
% ══════════════════════════════════════════════════════════
% Section 6 — Crossover Analysis (~2 pages)
% ══════════════════════════════════════════════════════════
\section{Crossover Analysis}
\label{sec:crossover}

The central question for \prism{} is: \emph{at what context length
does the photonic accelerator become favorable over electronic
alternatives?}
In this section we formalize the crossover condition and map the
favorable operating regime.

\subsection{Crossover Point Definition}
\label{sec:cross_definition}

We define the crossover point as the context length $n^*$ at which
the total cost of \prism{}-assisted decoding equals that of the
electronic baseline, for a given cost metric (energy or latency).

The total decode cost per token for a retrieval head consists of
two terms:
\begin{equation}
  C_{\text{total}} = C_{\text{select}}(n) + C_{\text{fetch}}(n, k),
  \label{eq:cost_total}
\end{equation}
where $C_{\text{select}}$ is the cost of determining which blocks
to fetch and $C_{\text{fetch}}$ is the cost of reading and computing
attention over the selected blocks.

For the \textbf{GPU full scan} baseline, no selection is needed
($k = N = n/B$), so
\begin{equation}
  C_{\text{GPU}} = C_{\text{fetch}}^{\text{GPU}}(n, n/B)
  = \frac{2\,d_h\,n\,b_{\text{prec}}}{\text{BW}_{\text{HBM}}},
  \label{eq:cost_gpu}
\end{equation}
where $\text{BW}_{\text{HBM}}$ is the HBM bandwidth
($\sim$\SI{3.2}{TB/s} for A100).

For \textbf{\prism{}}, the cost is
\begin{equation}
  C_{\text{PRISM}} = C_{\text{select}}^{\text{PRISM}}(n)
  + C_{\text{fetch}}^{\text{GPU}}(n, k\cdot B),
  \label{eq:cost_prism}
\end{equation}
where $C_{\text{select}}^{\text{PRISM}}$ is the dynamic energy of
the photonic evaluation (laser, DAC, modulator, PD, ADC):
\begin{equation}
  C_{\text{select}}^{\text{PRISM}} \approx E_{\text{dynamic}},
  \label{eq:cost_prism_select}
\end{equation}
Note that on the TFLN platform, the static MRR tuning power is
near zero (capacitive EO), so the selection cost is dominated
entirely by the dynamic components (${\sim}\SI{931}{pJ}$ per query,
\cref{tab:prism_energy}).
The fetch cost is reduced by the selection ratio $k/N$:
\begin{equation}
  C_{\text{fetch}}^{\text{GPU}}(n, k\cdot B)
  = \frac{2\,d_h\,k\,B\,b_{\text{prec}}}{\text{BW}_{\text{HBM}}}.
  \label{eq:cost_prism_fetch}
\end{equation}

The crossover occurs when $C_{\text{PRISM}} < C_{\text{GPU}}$,
i.e., when the memory bandwidth saved by not fetching $(N - k)$
blocks exceeds the cost of operating the photonic selector.

Setting $C_{\text{PRISM}} = C_{\text{GPU}}$ and solving for $n$
yields:
\begin{equation}
  n^* = \frac{C_{\text{select}}^{\text{PRISM}} \cdot
  \text{BW}_{\text{HBM}}}{2\,d_h\,b_{\text{prec}}\,(1 - k\,B/n^*)},
  \label{eq:crossover_implicit}
\end{equation}
which must be solved self-consistently since $k$ and $N = n/B$
both depend on $n$.
In practice, $k$ is a fixed parameter (e.g., $k = 32$), so the
selection ratio $k\,B/n \to 0$ as $n \to \infty$, and the crossover
simplifies to
\begin{equation}
  n^* \approx \frac{C_{\text{select}}^{\text{PRISM}} \cdot
  \text{BW}_{\text{HBM}}}{2\,d_h\,b_{\text{prec}}}.
  \label{eq:crossover_approx}
\end{equation}

\subsection{Results}
\label{sec:cross_results}

We evaluate the crossover across a three-dimensional parameter space:
context length $n \in [\num{4096}, \num{1000000}]$, signature
dimension $d \in [16, 128]$, and number of MRR banks
$N_{\text{bank}} \in [1, 16]$ (which controls the splitting loss
trade-off).

\begin{figure}[!htb]
  \centering
  \includegraphics[width=\columnwidth]{figures/fig_crossover_contour.pdf}
  \caption{%
    Energy crossover map for \prism{} vs.\ electronic baselines.
    The crossover contour (thick black line, $C_{\text{PRISM}} /
    C_{\text{baseline}} = 1$) shifts to shorter context lengths
    as signature dimension $d$ decreases (fewer MRRs, lower
    dynamic power).
    (a)~vs.\ GPU full scan: mathematical crossover at $n^* < 1$K
    tokens (TFLN), practical benefit at $n \geq 4$K;
    $n^* \approx 4$K tokens (SOI).
    (b)~vs.\ GPU ANN: crossover at $n^* \approx 2$K tokens.
    (c)~vs.\ NVIDIA ICMS: crossover at $n^* \approx 4$K tokens.
  }
  \label{fig:crossover_contour}
\end{figure}

\paragraph{Energy crossover.}
On the TFLN platform, the elimination of static heater power
dramatically shifts the crossover in \prism{}'s favor.
Against the GPU full scan baseline (\cref{fig:crossover_contour}a),
the mathematical crossover occurs at $n^* < 1$K tokens
for $d = 64$ and $N_{\text{bank}} = 4$; however, the practical
benefit emerges at $n \geq 4$K where block selection yields
meaningful traffic reduction ($>8\times$).
Below 4K the absolute memory traffic is already small enough that
photonic acceleration provides limited wall-clock improvement.
The \prism{} selection energy (${\sim}\SI{931}{pJ}$, entirely
dynamic) is five orders of magnitude below the GPU fetch energy
at 128K context (${\sim}\SI{48}{\micro\joule}$), making the photonic
selector effectively free in energy terms.

We note that this GPU baseline assumes a full-dimension scan
($d_h{=}128$); if the GPU instead scans compressed $d{=}32$
signatures in HBM, the scan energy drops to
$E_{\text{scan}}^{\text{fair}} = 2 \times 32 \times 1024 \times
2\;\text{B}\,/\,\SI{3.35}{TB/s} \approx \SI{12}{\micro\joule}$---a
$4\times$ reduction from the full-key baseline.
Even under this fairer comparison, \prism{}'s per-query energy
remains four orders of magnitude lower, preserving a comfortable
crossover margin.

This is a fundamental improvement over thermo-optic SOI platforms,
where the ${\sim}\SI{164}{\watt}$ heater power would place the
crossover at $n^* \approx 4$K tokens.

Against the GPU ANN baseline (FAISS IVF-PQ), which itself reduces
the electronic selection cost by $O(\sqrt{N})$, the crossover shifts
to $n^* \approx 2$K tokens---well below even moderate context lengths.

Against NVIDIA ICMS, which uses a DPU with lower memory bandwidth
than the GPU HBM, the crossover depends on the DPU's internal
bandwidth specification.
Using estimated values from the NVIDIA GTC 2024 announcement, the
crossover is at $n^* \approx 4$K tokens.

\paragraph{Latency crossover.}
The latency crossover is more favorable for \prism{} because the
$\sim$\SI{9}{\nano\second} photonic evaluation time is orders of
magnitude below the $\sim$\SI{5}{\micro\second} GPU scan.
Even including the ADC and top-$k$ overhead, \prism{} latency is
dominated by the subsequent KV block fetch from memory, making the
selection step effectively ``free'' in terms of latency.
The latency crossover therefore occurs at very short context lengths
($n^* \lesssim 4$K tokens).

\paragraph{Sensitivity analysis.}
We identify the dominant factors controlling the crossover:
\begin{enumerate}[leftmargin=*,itemsep=2pt]
  \item \textbf{Dynamic power} ($P_{\text{dynamic}}$):
    with TFLN EO tuning eliminating static heater power,
    the remaining power budget (${\sim}\SI{88}{\milli\watt}$)
    is dominated by TIAs, ADCs, and DACs.
    This is negligible compared to electronic baselines.
  \item \textbf{Signature dimension} ($d$):
    directly controls MRR count and hence chip area.
    There is a trade-off with recall quality
    (\cref{sec:sw_signature}).
  \item \textbf{Number of banks} ($N_{\text{bank}}$):
    affects splitting loss and laser power but also determines
    parallelism.
  \item \textbf{HBM bandwidth} ($\text{BW}_{\text{HBM}}$):
    improvements in electronic memory bandwidth (e.g., HBM4)
    will shift the crossover to longer contexts, raising the
    bar for photonic acceleration.
\end{enumerate}

\subsection{Scaling Projections}
\label{sec:cross_scaling}

As context lengths scale beyond current limits, the advantage of
\prism{} grows because electronic selection cost scales linearly
with $n$ (all signatures must be scanned) while \prism{} selection
cost is fixed (all signatures are pre-programmed in the weight bank).

\paragraph{Million-token contexts.}
At $n = \num{1000000}$ with $B = 128$, there are $N \approx 8000$
blocks.
The GPU full scan reads $8000 \times 64 \times 2 = \SI{1}{\mega\byte}$
of signature data per head per query.
The \prism{} weight bank accommodates this by using
$N_{\text{bank}} = 8$ banks of 1000 channels each, with a total of
$8 \times 1000 \times 64 = \num{512000}$ MRRs.
While the MRR count is large, the energy ratio
$C_{\text{PRISM}} / C_{\text{GPU}}$ decreases as $\sim 1/n$, making
the photonic approach increasingly favorable.

\paragraph{Multi-agent shared KV cache.}
In multi-agent scenarios where multiple LLM agents share a common
KV cache (e.g., retrieval-augmented agents querying the same
document store), a single \prism{} weight bank can serve multiple
agents simultaneously.
The block signatures are shared, and only the query sketch changes
per agent.
This amortizes the dynamic power over $A$ agents, reducing the
effective per-agent cost by $1/A$ and shifting the crossover to
even shorter context lengths.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=\columnwidth]{figures/fig_scaling_projection.pdf}
  \caption{%
    Scaling of energy advantage with context length.
    The energy ratio decreases as $\sim 1/n$ because the electronic
    scan cost grows linearly while \prism{} selection cost is fixed.
    At \num{1000000} tokens with $B = 128$ and $k = 8$, the traffic
    reduction reaches $977\times$, making \prism{} increasingly
    energy-efficient relative to GPU full scan.
  }
  \label{fig:scaling_projection}
\end{figure}


==> sections/software_analysis.tex <==
% ══════════════════════════════════════════════════════════
% Section 4 — Software Analysis (~2 pages)
% ══════════════════════════════════════════════════════════
\section{Software Analysis}
\label{sec:software}

This section presents the algorithmic evaluation of the \prism{}
candidate selection pipeline, independent of hardware impairments.
We profile retrieval heads, evaluate signature designs, and measure
recall and traffic reduction on real LLM workloads.

\subsection{Retrieval Head Identification}
\label{sec:sw_retrieval}

\paragraph{Models and datasets.}
We profile two representative open-weight LLMs:
Qwen2.5-7B-Instruct~\cite{Qwen2_2024} ($L=28$, $H=28$,
$d_h=128$, GQA with $H_{\text{KV}}=4$; total 112 KV heads) and
Qwen3-8B~\cite{Qwen3_2025} ($L=36$, $H=32$,
$d_h=128$, GQA with $H_{\text{KV}}=8$; total 288 KV heads).
Qwen2.5-7B supports context lengths of at least \num{128000} tokens;
Qwen3-8B supports up to \num{32000} tokens.
We compute retrieval ratios $R_h^{(\ell,h)}$ (\cref{eq:retrieval_ratio})
on a calibration set of 2--3 random token sequences per context length,
with $w = 256$ as the local window size.
The retrieval ratio is measured using a two-step procedure: SDPA-based
prefill followed by eager last-token attention extraction.
All experiments are run on an NVIDIA RTX 5880 (48\,GB VRAM) for
bf16 models, and an NVIDIA RTX 5070 (12\,GB) for 4-bit quantized
variants.
We additionally verify consistency between bf16 and 4-bit quantized
Qwen2.5-7B, finding that quantization does not substantially alter
retrieval head identification (e.g., 91.1\% vs.\ 92.0\% at 8K context
for bf16 and 4-bit, respectively).

\paragraph{Results.}
\Cref{fig:retrieval_heatmap} shows the retrieval ratio heatmap
across all layers and heads for both models.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=\columnwidth]{figures/fig_rh_heatmap.pdf}
  \caption{%
    Retrieval ratio $R_h^{(\ell,h)}$ for each KV head across
    all layers.
    Heads with $R_h > 0.3$ (dashed line) are classified as
    retrieval heads.
    (a)~Qwen2.5-7B: 102/112 heads are retrieval heads
    (91.1\%) at 8K context.
    (b)~Qwen3-8B: 258/288 heads are retrieval heads
    (89.6\%) at 8K context.
  }
  \label{fig:retrieval_heatmap}
\end{figure}

\Cref{tab:retrieval_vs_context} summarizes the retrieval head
fraction as a function of context length for both models.

\begin{table}[!htb]
  \centering
  \small
  \caption{%
    Retrieval head fraction at threshold $\tau = 0.3$ across context
    lengths. $R_h(\tau)$: percentage of KV heads with $R_h > \tau$.
    Mean $\bar{R}_h$: average retrieval ratio across all heads.
  }
  \label{tab:retrieval_vs_context}
  \begin{tabular}{@{}llccc@{}}
    \toprule
    Model & Context & $R_h(\tau{=}0.3)$ (\%) & Heads & Mean $\bar{R}_h$ \\
    \midrule
    \multirow{7}{*}{Qwen2.5-7B}
      & 2K   & 83.9 & 94/112  & 0.574 \\
      & 4K   & 83.0 & 93/112  & 0.560 \\
      & 8K   & 91.1 & 102/112 & 0.627 \\
      & 16K  & 92.9 & 104/112 & 0.639 \\
      & 32K  & 95.5 & 107/112 & 0.656 \\
      & 65K  & 92.0 & 103/112 & 0.633 \\
      & 128K & 98.2 & 110/112 & 0.796 \\
    \midrule
    \multirow{3}{*}{Qwen3-8B}
      & 2K  & 86.5 & 250/288 & 0.626 \\
      & 4K  & 88.2 & 254/288 & 0.652 \\
      & 8K  & 89.6 & 258/288 & 0.657 \\
    \bottomrule
  \end{tabular}
\end{table}

We observe the following patterns:
\begin{itemize}[leftmargin=*,itemsep=2pt]
  \item \textbf{Ubiquity of retrieval behavior.}
    At a threshold of $\tau = 0.3$, 91.1\% of KV heads in Qwen2.5-7B
    and 89.6\% in Qwen3-8B are retrieval heads at 8K context.
    This prevalence increases with context length: for Qwen2.5-7B,
    the fraction rises from 83.9\% at 2K to 98.2\% at 128K context,
    indicating that nearly all heads engage in long-range retrieval
    at long contexts.
    Note that at the more permissive $\tau = 0.1$ threshold used
    in~\cite{DuoAttention2024}, essentially 100\% of heads qualify
    as retrieval heads.
  \item \textbf{Layer distribution.}
    Analysis of the highest-scoring retrieval heads in Qwen2.5-7B
    reveals concentration in middle-to-late layers (layers 14--26),
    with isolated early-layer exceptions (e.g., L4H1 with $R_h = 0.965$).
    The top retrieval heads include L4H1 (0.965), L14H0 (0.939),
    L24H3 (0.938), L22H3 (0.938), L22H0 (0.936), L26H0 (0.923),
    and L25H1 (0.921), suggesting that the model develops specialized
    long-range attention patterns predominantly in deeper layers.
  \item \textbf{GQA effect.}
    Because GQA shares KV heads across multiple query heads, the
    number of \emph{KV cache entries} requiring retrieval-style
    treatment is even smaller than the head count suggests.
\end{itemize}

The key implication for \prism{} is that the photonic accelerator
needs to serve the vast majority of KV heads---102 out of 112
for Qwen2.5-7B and 258 out of 288 for Qwen3-8B at 8K context.
However, GQA sharing means each KV head serves multiple query heads,
so the \emph{number of independent weight bank instances} required
equals the KV head count, not the query head count.

\subsection{Block Partitioning and Signature Generation}
\label{sec:sw_signature}

We partition the KV cache into contiguous blocks of $B$ tokens
and compute a $d$-dimensional signature for each block.
We evaluate mean-key and random projection signature methods
from \cref{sec:arch_signature} at block size $B = 128$ and
signature dimensions $d \in \{16, 32, 64, 128\}$,
using Qwen2.5-7B at context length $n = 4096$.
Our experiments identify $B = 128$ with $d = 32$ and mean-key
projection as the best configuration, achieving Recall@8 = 77.3\%
(R@2 = 31.3\%, R@4 = 50.0\%).
Mean-key projection consistently outperforms random projection
across all tested dimensions, confirming that the natural key-space
geometry contains exploitable structure for block ranking.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=\columnwidth]{figures/fig_recall_comparison.pdf}
  \caption{%
    Recall@$k$ as a function of signature dimension $d$
    for different signature methods.
    Block size $B = 128$, top-$k = 8$ (0.8\% of blocks
    at $n = \num{128000}$).
    Mean-key projection consistently outperforms random projection,
    achieving 77.3\% recall@8 at $d = 32$.
  }
  \label{fig:recall_vs_dim}
\end{figure}

\paragraph{Non-negative encoding.}
Since MRR weights are physically constrained to $[0, 1]$, we
compare two non-negative encoding strategies:
(i)~\emph{split encoding}, which represents each signed component
as two non-negative halves ($\sigma^+$ and $\sigma^-$), effectively
doubling the dimension to $2d$; and
(ii)~\emph{ReLU projection}, which applies $\vect{\sigma} =
\max(0, \mat{R}\,\bar{\vect{k}})$.
We find that ReLU projection with dimension $d$ achieves recall
comparable to split encoding at dimension $d/2$, while requiring
half the MRR count.

\subsection{Recall and Traffic Reduction}
\label{sec:sw_recall}

We define recall@$k$ as the fraction of the true top-$k$ blocks
(by exact query--key inner product) that appear in the \prism{}-selected
top-$k$ blocks:
\begin{equation}
  \text{Recall@}k = \frac{|\mathcal{S}_{\text{PRISM}} \cap
    \mathcal{S}_{\text{exact}}|}{k},
  \label{eq:recall}
\end{equation}
where $\mathcal{S}_{\text{PRISM}}$ and $\mathcal{S}_{\text{exact}}$
are the sets of top-$k$ block indices selected by \prism{} and by
exact computation, respectively.

\begin{table}[!htb]
  \centering
  \small
  \caption{%
    Recall@$k$ for \prism{} block selection.
    Qwen2.5-7B, $n = 4096$, mean-key projection.
    Traffic ratio: $k \cdot B / n$ at $n = \num{128000}$.
  }
  \label{tab:recall_params}
  \begin{tabular}{@{}ccccccc@{}}
    \toprule
    $B$ & $d$ & $k$ & R@2 (\%) & R@4 (\%) & R@8 (\%) & Traffic$_{128\text{K}}$ (\%) \\
    \midrule
    128 & 32  & 2/4/8  & 31.3 & 50.0 & 77.3 & 0.8 \\
    \bottomrule
  \end{tabular}
\end{table}

Traffic reduction is defined as the ratio of fetched KV cache bytes
to the full cache size:
\begin{equation}
  \text{Traffic ratio} = \frac{k \cdot B \cdot 2 d_h \cdot
    b_{\text{prec}}}{n \cdot 2 d_h \cdot b_{\text{prec}}}
  = \frac{k \cdot B}{n}.
  \label{eq:traffic_reduction}
\end{equation}
At $n = \num{128000}$, $B = 128$, $k = 8$, the traffic ratio is
$8 \times 128 / \num{128000} = 0.8\%$---a $125\times$ reduction
in memory bandwidth demand.
At million-token scale ($n = \num{1000000}$), the same parameters
yield a traffic ratio of $8 \times 128 / \num{1000000} = 0.1\%$,
or a $977\times$ reduction.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=\columnwidth]{figures/fig_traffic_reduction.pdf}
  \caption{%
    Memory traffic reduction factor as a function of context length
    for fixed block size $B = 128$ and $k = 8$ selected blocks.
    The traffic reduction scales linearly with context length,
    reaching $977\times$ at $n = \num{1000000}$.
  }
  \label{fig:traffic_reduction}
\end{figure}

\subsection{Downstream Quality: Relationship to Existing Methods}
\label{sec:sw_downstream}

The block-level top-$k$ selection mechanism at the core of \prism{}
is not a novel algorithmic contribution---several recent works have
demonstrated that block-level KV-cache selection preserves downstream
task quality.
Quest~\cite{Quest2024} shows that selecting the top-$k$ KV pages
(blocks) by query--key inner product maintains over 99\% of full
attention accuracy on a range of long-context benchmarks, including
Needle-in-a-Haystack (NIAH) with perfect retrieval accuracy up to
1M tokens.
DuoAttention~\cite{DuoAttention2024} demonstrates that distinguishing
retrieval heads from streaming heads and applying sparse attention
only to retrieval heads preserves LongBench performance within 1--2\%
of full attention.
InfLLM~\cite{InfLLM2024} and RocketKV~\cite{RocketKV2024} provide
additional evidence that block-level selection is a sound strategy
for long-context inference.

Our contribution is orthogonal: we focus on whether the block
selection quality is maintained when the similarity computation---the
inner product between the query sketch and block signatures---is
performed by a \emph{realistic photonic MRR array} rather than
digital hardware.
The key question is not ``does block selection preserve quality?''
(answered affirmatively by the works above) but rather ``does
MRR-based analog computation introduce sufficient error to degrade
the selection, and if so, under what physical parameter regimes?''

To address this question, we evaluate \prism{} in two modes:
\begin{enumerate}[leftmargin=*,itemsep=2pt]
  \item \textbf{Software baseline}: exact (FP32) inner-product
    block selection, establishing the recall and NIAH accuracy
    achievable with ideal computation.
  \item \textbf{MRR-simulated}: block selection using the MRR weight
    bank model (\cref{sec:hw_impairments}), with FDTD-calibrated
    physical impairments including quantization, thermal drift,
    insertion loss, crosstalk, and detector noise.
\end{enumerate}

\paragraph{Needle-in-a-Haystack validation.}
We validate that \prism{} block selection correctly retrieves the
``needle'' block across context lengths from \num{4096} to
\num{128000} tokens, comparing full attention, software-selected,
and MRR-selected attention.
The NIAH experiment directly tests whether the photonic hardware's
ranking errors cause the needle block to fall outside the top-$k$
selection, which would manifest as a retrieval failure.
Results of this comparison are presented in \cref{sec:hw_impairments},
where the MRR impairment parameters are varied systematically.

